GODS: Generalized One-class Discriminative Subspaces for Anomaly Detection

One-class learning is the classic problem of fitting a model to data for which annotations are available only for a single class. In this paper, we propose a novel objective for one-class learning. Our key idea is to use a pair of orthonormal frames -- as subspaces -- to "sandwich" the labeled data via optimizing for two objectives jointly: i) minimize the distance between the origins of the two subspaces, and ii) to maximize the margin between the hyperplanes and the data, either subspace demanding the data to be in its positive and negative orthant respectively. Our proposed objective however leads to a non-convex optimization problem, to which we resort to Riemannian optimization schemes and derive an efficient conjugate gradient scheme on the Stiefel manifold. To study the effectiveness of our scheme, we propose a new dataset~\emph{Dash-Cam-Pose}, consisting of clips with skeleton poses of humans seated in a car, the task being to classify the clips as normal or abnormal; the latter is when any human pose is out-of-position with regard to say an airbag deployment. Our experiments on the proposed Dash-Cam-Pose dataset, as well as several other standard anomaly/novelty detection benchmarks demonstrate the benefits of our scheme, achieving state-of-the-art one-class accuracy.

==> kgods.tex <==
\section{Kernelized GODS}
In this section, we formulate a kernelized variant of the GODS algorithm. Let us reconsider our GODS formulation in Eq. 9. To simplify our notation, we avoid the slack variables and assume the bias variables $\vb$ are included in the inputs $\vx$.  Then, we can rewrite the formulation P3 ( in the main paper) as:
\begin{align}
    \min_{\mW_1,\mW_2\in\stiefel{K}} & \half\sum_{i=1}^n \enorm{\mW_1^T\vx_i}^2 + \enorm{\mW_2^T\vx_i}^2\notag\\
    \subjectto & \min(\mW_1^T\vx_i) \geq \eta, \quad\forall i\in\indexset{n}\notag\\
    &\max(\mW_2^T\vx_i) \leq \eta, \quad\forall i\in\indexset{n},
    \label{eq:p1}
\end{align}
where we denote $\indexset{n}$ as the index set. Let us for now drop the Stiefel manifold constraints on the weight matrices, and further let us rewrite the constraints in the standard form:
\begin{align}
    \min_{\mW_1,\mW_2} & \half\sum_{i=1}^n \enorm{\mW_1^T\vx_i}^2 + \enorm{\mW_2^T\vx_i}^2\notag\\
    \subjectto\quad &\eta - \mW_{1j}^T\vx_i \leq 0,\quad\forall j\in\indexset{K}, i\in\indexset{n}\notag\\
    &\mW_{2j}^T\vx_i - \eta \leq 0,\quad\forall j\in\indexset{K}, i\in\indexset{n}.
    \label{eq:p2}
\end{align}
In~\eqref{eq:p2}, we assume $\mW_{1j}$ represents the $j$-th column of $\mW_1$. Now, we need some more notation. Let $\mX$ be a $d\times n$ matrix obtained by stacking each data point $\vx_i$ along its column. Then, by introducing non-negative Lagrangian multipliers $\mY,\mZ\in\realsp{K\times n}$, we can write the Lagrangian $L(\mW_1,\mW_2, \mY, \mZ)$ of~\eqref{eq:p2} as:
\begin{align}
L :=& \half\trace{\mW_1\mW_1^T\mX\mX^T} + \half\trace{\mW_2\mW_2^T\mX\mX^T} \notag\\
& + \trace{\mZ^T\left(\eta\one_{K\times n} - \mW_1^T\mX\right)} \notag\\
& + \trace{\mY^T\left(\mW_2^T\mX -\eta\one_{K\times n}\right)},
\label{eq:3}
\end{align}
where $\one_{K\times n}$ is a $K\times n$ matrix of all ones. Expressing the primals in terms of the multipliers yields $\mW_1=\inv{\mX\mX^T}\mX\mZ^T$ and $\mW_2=-\inv{\mX\mX^T}\mX\mY^T$. Substituting the variables into the Lagrangian, and making some straightforward reductions and simplifications, we have the following dual formulation:
\begin{align}
    \min_{\mY,\mZ\in\realsp{K\times n}} &  \half\trace{\mY\kernel\mY^T + \mZ\kernel\mZ^T}
    -\eta\one_K^T\left(\mY-\mZ\right)\one_n\notag\\
    & \text{where }\kernel = \mX^T\inv{\mX\mX^T}\mX.
    \label{eq:4}
\end{align}

Recall that we had dropped the manifold constraints in the above derivations, which are $\mW_1^T\mW_1=\mW_2^T\mW_2=\eye{K}$. Substituting for these in the dual form, we have the following manifold constraints on the dual variables as:
\begin{align}
    \mZ\pp\mZ^T = \mY\pp\mY^T = \eye,
\end{align}
where $\pp=\mX^T\left(\mX\mX^T\right)^{-2}\mX$. We can consolidate the above expressions and write the complete dual formulation, which we call K-GODS as:
\begin{align}
    \min_{\mY,\mZ\in\realsp{K\times n}} &  \half\trace{\mY\kernel\mY^T + \mZ\kernel\mZ^T}
    -\eta\one_K^T\left(\mY-\mZ\right)\one_n\notag\\
    &\mZ\pp\mZ^T = \mY\pp\mY^T = \eye{K}.
    \label{eq:kgods}
\end{align}
Similar to the Stiefel manifold corresponding to the orthogonality constraints on the primal problem, the constraints in~\eqref{eq:kgods} put the optimization on a \emph{generalized Stiefel manifold} (assuming $\pp$ is positive definite)~\cite{edelman1998geometry,Cherian_2018_CVPR}, and can be solved using manifold optimization techniques via popular solvers such as ManOpt~\cite{boumal2014manopt}.





==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}
Due to the significant practical utility of one-class model, they have been explored in great depth in a variety of disciplines including but not limited to remote sensing~\cite{matteoli2014overview}, network intruder detection~\cite{lazarevic2003comparative}, and fraud detection~\cite{heller2003one}. In computer vision, one-class classifiers are popularly used for anomaly detection such as for example in surveillance videos~\cite{del2016discriminative,popoola2012video,saligrama2012video}, medical imaging~\cite{krawczyk2015one}, or finding anomalous object attributes in image sets~\cite{saleh2013object}. For a comprehensive review of applications on this topic, we refer the interested reader to excellent surveys such as~\cite{chandala2009anomaly,pimentel2014review}.


% In general, anomaly detection is to identify the test data points that are not fitting the normal data distribution from the training set~\cite{schlegl2017unsupervised}. It is an actively and heavily researched topic and exist in various areas, such as video analysis~\cite{del2016discriminative}, remote sensing~\cite{matteoli2014overview}, and cyber-security~\cite{chandala2009anomaly}. In the area of computer vision, the works are mainly focus on video-based anomaly detection for finding the abnormal motion or object from the surveillance video~\cite{popoola2012video,saligrama2012video}. Or the image-based object anomaly detection for identifying both anomalies and anomaly attribute from the image set~\cite{saleh2013object}.  

In computer vision, anomaly detection has been looked at from several facets. In Adam et al.,~\cite{adam2008robust} and Kim et al.~\cite{kim2009observe}, optical flow is used to capture motion dynamics on which a discriminative model is built for detecting anomalies. Gaussian mixture modelling of people and object trajectories is used in~\cite{li2013visual,sillito2008semi} for anomaly detection in video sequences. Saliency is used in~\cite{itti2000saliency,judd2009learning}. Detecting out-of-context objects is explored in~\cite{choi2012context, park2012abnormal} using support graph and generative models for characterizing normal and abnormal data. Compactness and discriptiveness losses are used in~\cite{perera2018learning} for training neural nets for anomaly detection. 
% Based on different scenarios, several typical algorithms have been developed for learning the feature representation. To build model upon optical flow are usually found to be useful to capture the motion dynamic and is discriminative for detecting the anomalies~\cite{adam2008robust,kim2009observe}. Building Gaussian Mixture Models(GMM) or Support Vector Machine(SVM) on the trajectory of object and person is another popular method~\cite{li2013visual,sillito2008semi}, which capture both spatial and temporal information of the video sequence. Detecting salient regions in images has also been implemented by some researchers~\cite{itti2000saliency,judd2009learning}. Recently, out-of-context objects have been emphasis by~\cite{choi2012context,park2012abnormal}, who use support graph and generative model for characterizing the normality and abnormality. Besides, neural network is also found to be useful in~\cite{perera2018learning}, which introduce compactness and descriptiveness loss during the training.

% However, the most methods discussed so far are about feature learning and embedding, which help us to well model the data points. To finish the binary classification, one-class classifier will be introduced in the next, and rare novel work has been found in designing such classifier. Thus, in this paper, we propose a new one-class formulation based on the traditional one-class classifier, aiming to solve different one-class problems including the anomaly detection task. One recent work share the similar motivation as ours, which introduce subspace representation scheme to describe the data points~\cite{sohrab2018subspace}. Raghavendra et.al also propose OC-NN to learn the one-class classifier inside the neural network by data driven~\cite{chalapathy2018anomaly}. Compared with our scheme, their formulation and problem set-up are totally different.

% Like anomaly detection, novelty detection and outlier explanation are also sub-tasks of one-class classification problem. And in this area, One-Class Support Vector Machine (OC-SVM) and Support Vector Domain Description (SVDD) are two of the most popular methods, which will be briefly introduced in the next section, combined with the evolution of our scheme.
